VoDaSuRe: A Large-Scale Dataset Revealing Domain Shift in Volumetric Super-Resolution

Recent advances in volumetric super-resolution (SR) have demonstrated strong performance in medical and scientific imaging, with transformer- and CNN-based approaches achieving impressive results even at extreme scaling factors. In this work, we show that much of this performance stems from training on downsampled data rather than real low-resolution scans. This reliance on downsampling is partly driven by the scarcity of paired high- and low-resolution 3D datasets. To address this, we introduce VoDaSuRe, a large-scale volumetric dataset containing paired high- and low-resolution scans. When training models on VoDaSuRe, we reveal a significant discrepancy: SR models trained on downsampled data produce substantially sharper predictions than those trained on real low-resolution scans, which smooth fine structures. Conversely, applying models trained on downsampled data to real scans preserves more structure but is inaccurate. Our findings suggest that current SR methods are overstated - when applied to real data, they do not recover structures lost in low-resolution scans and instead predict a smoothed average. We argue that progress in deep learning-based volumetric SR requires datasets with paired real scans of high complexity, such as VoDaSuRe. Our dataset and code are publicly available through: https://augusthoeg.github.io/VoDaSuRe/

==> sec/1_intro.tex <==
\begin{comment}

\section{Introduction}
\label{sec:intro}

Volumetric super-resolution promises to reveal details hidden in 3D scans -- but are today’s deep learning models truly reconstructing reality, or just reversing a downsampling operation?

Deep learning-based volumetric super-resolution (SR) has achieved remarkable progress in recent years. However, as we demonstrate, much of this success is an artifact of the training data rather than true predictive capability. The dominant approach relies on paired high- and low-resolution volumes, where the low-resolution volumes are generated by downsampling high-resolution scans \cite{}. This setup produces near-perfect predictions, but only because the models learn to invert a deterministic downsampling process on relatively simple data.

When trained on real and complex data, i.e., volumes recorded at both high and low resolutions and fine structures, the story changes dramatically. Predictions become smeared and lose fine structural details, far from the sharp reconstructions seen with downsampled data as illustrated in \cref{fig:overview_vodasure}.

\begin{figure}[t]
   \centering
   \includegraphics[width=1.0\linewidth]{example-image-a}
   \caption{Overview of \datasetname}
   \label{fig:overview_vodasure}
\end{figure}

To investigate this discrepancy, we introduce \textbf{VoDaSuRe} -- \textbf{Vo}lumetric \textbf{Da}taset for \textbf{Su}per-\textbf{Re}solution, a large-scale CT dataset specifically designed for SR research. \datasetname includes samples scanned at multiple resolutions using the same micro-CT scanner, along with downsampled versions for direct comparison.

Using \datasetname, we trained models under two conditions: 1) Scanned low-resolution data to high-resolution prediction. 2) Downsampled data to high-resolution prediction. The difference is significant: models trained on downsampled data recover fine structures accurately, while models trained on scanned low-resolution data produce severely smeared predictions. Surprisingly, applying downsample-trained models to real low-resolution scans preserves more structure than models trained on scanned data, but still lacks precision compared to predictions from downsampled inputs. These findings point to a significant domain shift between scanned and downsampled data and highlight the need for further research in volumetric SR, now enabled by \datasetname.

\datasetname spans a wide range of structural complexity, including wood, wood composites, cardboard, and bone (bovine and human). Bone volumes are relatively simple, with high contrast and smooth variations, whereas wood-based samples exhibit coarse to extremely fine structures, ranging from regular solid wood to chaotic fiber composites.

Critically, fine canal structures in wood vanish at low resolution and cannot be recovered by models trained on scanned data, which instead predict smeared averages. In contrast, models trained on downsampled data reconstruct these structures, even when they are absent in the low-resolution input. This behavior suggests that current SR models do not truly infer missing structures but rather learn to reverse synthetic degradation. The distribution shift between scanned and downsampled data underscores the limitations of existing SR approaches and motivates the need for datasets like \datasetname to drive progress toward clinically and scientifically relevant solutions.

A desired property of SR used for volumetric data is to predict structures with the same properties as the high-resolution training data, ensuring the data distribution remains the same. Specifically, for the \datasetname wood samples, the SR models should ideally predict the canal structures seen in the high-resolution wood samples, also in regions where these canals are not visible in the low-resolution data. As highlighted in \cref{fig:overview_vodasure}, current state-of-the-art models do not predict structures with the same properties. Instead, they predict a smeared average, where details are lost.

Although most data is not medical, SR methods developed from \datasetname will be still be clinically relevant. The structures present in the samples scanned in \datasetname have great variation and much finer details than what is seen in datasets typically used for training SR models. The resolution of clinical scanners has greatly increased, especially CT scanners with photon counting detectors \cite{greffier2025photon,quintiens2024photon} and cone beam CT scanners \cite{ko2024role,siddall2024emerging,yu2022clinical}. With these scanners, details in both soft tissue and bone become visible, resulting in images with a structural variation resembling that of \datasetname. Furthermore, there is an increased use of micro-CT and synchrotron CT for scientific studies, which are the scanning modalities used to create \datasetname.

Our contributions are:
\begin{itemize}
    \item We introduce \datasetname, a volumetric SR dataset scanned at multiple resolutions. 
    \item We benchmark several state-of-the-art (SOTA) 2D and volumetric SR methods, including CNN- and ViT-based architectures across several volumetric datasets, including medical imaging datasets and our proposed \datasetname. Our experiments show that models trained and evaluated on downscaled volumes outperform compared to models trained and evaluated in a real setting where volumes scanned at low resolution.  
    \item We implement a custom volumetric image data pipeline designed for efficient out-of-core sampling of 3D patches.
    \item Our dataset and data pipeline are publicly available. 
\end{itemize}

\end{comment}

\section{Introduction}
\label{sec:intro}

Volumetric super-resolution promises to reveal details hidden in 3D scans, but are today’s deep learning models truly reconstructing missing high-resolution details, or merely learning to reverse synthetic downsampling?

Recent advances in deep learning-based volumetric super-resolution (SR) have achieved impressive results. However, we show that much of this success is a consequence of the training setup rather than genuine predictive capability. The dominant paradigm uses paired high- and low-resolution volumes, where the low-resolution volumes are generated by downsampling high-resolution scans \cite{}. This setup yields near-perfect reconstructions because models learn to invert a deterministic degradation process. Furthermore, the standard datasets are already relatively smooth and easy to super-resolve.

When trained on real low-resolution scans, i.e., volumes recorded at different resolutions, the story changes dramatically. Predictions become smeared and lose fine structural details, far from the sharp reconstructions observed with downsampled data (\cref{fig:intro_overview_vodasure}). This discrepancy raises a critical question: can current SR methods recover structures that vanish at low resolution, or do they simply predict plausible averages?

\begin{figure}[t]
   \centering
   \def\svgwidth{\linewidth}
    \input{figs/introfig/introfig.pdf_tex}
   %\includegraphics[width=1.0\linewidth]{example-image-a}
   \caption{Example from \datasetname: (a) volume of bamboo showing the cropped area in red, (b) high resolution crop, (c) 4$\times$ downsampled, (d) scan at 4$\times$ lower resolution, (e) SR of bamboo, (f) SR of cardboard. The top row in (e) and (f) is trained on downsampled HR-LR pairs, and the bottom row is trained on different resolution recordings.}
   \label{fig:intro_overview_vodasure}
\end{figure}

To address this, we introduce \textbf{VoDaSuRe} -- the \textbf{Vo}lumetric \textbf{Da}taset for \textbf{Su}per-\textbf{Re}solution -- a large-scale CT dataset designed for SR research. \datasetname contains samples scanned at multiple resolutions using the same micro-CT scanner, along with downsampled versions for benchmarking. Using \datasetname, we trained models under two conditions:  
(1) scanned low-resolution $\rightarrow$ high-resolution prediction, and  
(2) downsampled $\rightarrow$ high-resolution prediction.  

The results reveal a striking domain shift: models trained on downsampled data recover fine structures accurately, while models trained on scanned low-resolution data produce severely smeared predictions. Surprisingly, applying downsample-trained models to real low-resolution scans preserves more structure than models trained on scanned data, but still lacks precision compared to predictions from downsampled inputs. These findings highlight the limitations of current SR approaches and the need for datasets like \datasetname to enable clinically and scientifically relevant progress.

\datasetname spans diverse structural complexity, including wood, wood composites, cardboard, and bone (human and animal). Bone volumes exhibit high contrast and smooth variations, whereas wood-based samples range from regular solid wood to chaotic fiber composites with extremely fine canal structures. Critically, these canals vanish at low resolution and cannot be recovered by models trained on scanned data, which instead predict smeared averages. In contrast, models trained on downsampled data reconstruct these structures, even when absent in the input, suggesting that current SR models learn to reverse synthetic degradation rather than infer missing details.

Although most samples are non-medical, SR methods developed using \datasetname remain clinically relevant. Modern CT scanners, including photon-counting detectors \cite{greffier2025photon,quintiens2024photon} and cone-beam CT systems \cite{ko2024role,siddall2024emerging,yu2022clinical}, now capture fine details in bone and soft tissue, producing structural variation similar to \datasetname. Furthermore, micro-CT and synchrotron CT, used to create \datasetname, are increasingly employed in scientific studies. \textbf{Our contributions are:}
\begin{itemize}
    \item We introduce \datasetname, a large-scale volumetric SR dataset with paired high- and low-resolution scans and downsampled versions.
    \item We benchmark state-of-the-art CNN- and ViT-based SR methods across multiple volumetric datasets, including medical imaging and \datasetname, revealing significant performance gaps between synthetic and real low-resolution settings.
    \item We implement an efficient volumetric data pipeline for out-of-core sampling of 3D patches.
    \item We release \datasetname and our pipeline publicly to enable reproducible research.
\end{itemize}


\begin{comment}
\begin{table*}[t]
\renewcommand{\arraystretch}{1.00}
\centering
\begin{scriptsize}
\begin{NiceTabularX}{\textwidth}{XXXXXXXX}[hlines]
\toprule
Dataset & \#samples & \#volumes & Volume shape & Domain & Modalities & Accessibility & Multi-resolution \\
\midrule
% Example rows
% BrainMRI & 10k & 100 & $256^3$ & Medical & MRI & Public & Yes \\
% WoodCT & 500 & 10 & $512^3$ & Material & CT & Private & No \\
\bottomrule
\end{NiceTabularX}
\end{scriptsize}
\caption{Overview of image datasets featuring paired volumetric data.}
\label{tab:dataset_table}
\end{table*}
\end{comment}

\begin{table*}[t]
\renewcommand{\arraystretch}{1.00}

\begin{subtable}[t]{\linewidth}
\centering
\begin{scriptsize}
%\resizebox{\textwidth}{!}{%
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}cccccccc@{}}
\toprule
Dataset & \#samples & \#voxels & Volume shape & Domain & Modalities & Accessibility & Multi-resolution \\ \midrule
% Tilføj no. of pixels in total 
NAMIC \cite{NAMIC_wiki} & 20 & $\sim0.2\times 10^{9}$ & $256\times256\times176$ & Brain MRI & T1w, T2w, fMRI, DTI & On request & \xmark \\ 
Kirby 21 \cite{Landman_Kirby21_dataset} & 21 & $\sim0.3\times 10^{9}$ & $256\times256\times180$ & Brain MRI & T2w, FLAIR, DTI & Public & \xmark \\ 
IXI\footnote{\url{https://brain-development.org/ixi-dataset/}} & 600 & $\sim5.9\times 10^{9}$ & $256\times256\times(144\text{-}150)$ & Brain MRI & T1w, T2w, PD & Public & \xmark \\ 
%ADNI & - & - & $-$ & Brain MRI (Alzheimer's) & - & - & \xmark \\ 
fastMRI \cite{zbontar2018fastmri} & 8400 & $\sim11.0\times 10^{9}$ & $256\times256\times20$ (mean) & Brain \& knee MRI & T1w, T2w, FLAIR & Public & \xmark \\ 
BraTS 2023 \cite{Menze_BraTS_GLI} & 1470 & $\sim13.1\times 10^{9}$ & $240\times240\times155$ & Brain MRI (Glioma) & T1w, T2w & On request & \xmark \\ 
LiTS \cite{bilic_LITS} & 130 & $\sim17.4\times 10^{9}$ & $512\times512\times(0\textbf{-}987)$ & Liver CT & Clinical CT & Public & \xmark \\ 
HCP 1200 \cite{Van_HCP_1200_dataset} & 1113 & $\sim29.2\times 10^{9}$ & $320\times320\times256$ & Brain MRI & T1w, T2w & Public & \xmark \\ 
LIDC-IDRI \cite{Armato_LIDC_IDRI} & 1010 & $\sim104.3\times 10^{9}$ & $512\times512\times(65\textbf{-}764)$ & Thorax CT & Clinical CT & Public & \xmark \\ 
CTSpine1K \cite{deng_CTSpine1K} & 1005 & $\sim134.9\times 10^{9}$ & $512\times512\times(349\textbf{-}659)$ & Spine CT & Clinical CT & Public & \xmark \\ 

\midrule
\citet{solidbattery2023} & 1 (2) & $\sim0.1\times 10^{9}$ & $ 512 \times 512 \times 200$ & Materials & Lab- \& synchrotron CT & On request &  \cmark \\ 
\citet{li2022deep} & 61 (122) & $\sim0.9\times 10^{9}$ & $512 \times 512 \times 28$ & Brain MRI & T1w, T2w, FLAIR & On request &  
\cmark \\
\citet{chu2025paired} & 20 (40) & $\sim2.2\times 10^{9}$ & $480 \times 512 \times 224$ & Brain MRI & T1w, T2w & Unavailable &  
\cmark \\
WAND \cite{mcnabb2025wand} & 170 (846) & $\leq19.4\times 10^{9}$ & $\leq 320\times320\times224$ & Brain MRI & T1w, T2w, fMRI, TRUST & Public &  \cmark \\ 
\citet{klos2025super} & 1 (6) & $\sim20.5\times 10^{9}$ & $1181\times 1695\times 1695$ (mean) & Materials & Lab-CT & Public &  
\cmark \\ 
RPLHR-CT \cite{RPLHR_CT} & 250 (500) & $\sim52.0\times 10^{9}$ & $512 \times 521\times(191\text{-}396)$ & Thorax CT & Clinical CT & On request &  \cmark \\ 
I13-2 XCT \cite{green2025three} & 1 (4) & $\sim53.2\times 10^{9}$ & $2510\times2510\times2110 $ & Materials & Synchrotron CT & Public &  \cmark \\ 
FACTS \cite{Bardenfleth_FACTS} & 13 (26) & $\sim57.6\times 10^{9}$ & $1014 \times 1372 \times 1584$ (mean) & Femur CT & Lab- \& clinical CT & Public &  \cmark \\ 
%LDCT & - & - & $-$ & - & - & Public &  \xmark \\ 

\midrule
VoDaSuRe (ours) & 16 (32) & $\sim\underline{211.6 \times10^{9}}$ & $3454 \times 1948 \times 1926$ (mean)\footnote{The volume shape of the samples in VoDaSuRe varies, however all HR scans are chunked in cubes of $160^3$ voxels.}  & Medical/Materials & Lab CT & Public &  \cmark \\ 
\bottomrule
\end{tabular*}
%}%
\end{scriptsize}
\label{tab:ablation_levels}
\end{subtable}

\caption{Overview of volumetric image datasets, including single-resolution and paired multi-resolution datasets.}
\label{tab:dataset_table}
\end{table*}
%\end{comment}

\begin{comment}

 - Volumetric super-resolution is dominated by medical imaging datasets acquired using either CT or MRI.
 - Unlike 2D image dataset, which are usually designed to contain a broad range of items and features to ensure general applicability for a variety of method developments, 3D image datasets are usually very specialized. They are typically designed to address a specific problem, for instance the Brain Tumor Segmentation Challenge (BraTS) which primary focus is segmentation of brain lesions. Another dataset is CirrMRI600+, which is focused on segmentation of patients suffing with cirrhotic liver disease. Such datasets contain a very narrow range of unique image features. 
 - Volumetric image datasets are difficult to acquire, requiring complex acqusition setups as well as expert knowledge to obtain good results. Large scan times means higher effort to acquired each image instance with compared with 2D images, which can be found online. Moreover, the amount of data consumed by a volumetric image is difficult to handle computationally, further hindering the availablility of such datasets.  
 - Due to volumetric image datasets being sparsely available compared with 2D image datasets, volumetric image processing techniques are usually evaluated using a single dataset, as opposed to 2D approaches where datasets are abundant. Because of this combination of small number of available 3D datasets plus methods being evaluated sometimes on a single dataset, it is difficult to benchmark volumetric imaging methods confidently. 
 - There is a debate within the volumetric imaging community whether CNNs or ViTs are better for volumetric image processing. Seminal works such as nnUNet showed that CNN usually beat ViTs in volumetric segmentation tasks, however, all evaluations was done using medical imaging datasets. In volumetric super-resolution, recent findings show that the performance discrepancy of CNNs vs. ViTs depends on the dataset, with higher resolution 3D image domains favoring ViTs and CNNs being favored in lower-resolution image domains such as brain MRI. 

 - Apart from the lack of volumetric image datasets with diverse image features, there is a definite need for volumetric datasets specifically designed for super-resolution. In 2D, state-of-the-art super-resolution models are dominated by ViTs trained on vast datasets (ImageNet, DIV2K, Flicker, etc.). Because of this, they are generally applicable within the domain of 2D images. However, such datasets do not currently exist for volumetric super-resolution, which mostly use datasets of brain MRI and clinical CT scans.   
 - By far the most widespread practice for obtaining LR-HR image pairs in both 2D and volumetric super-rsolution is to use some type of degradation model to synthetically degrade the HR image to obtain a corresponding LR image. As state-of-the-art super-resolution frameworks rely on supervised training where correspondence between the LR and HR image is assumed, degradation models are convienient as one does not have to deal with image registration. However, such approaches are not realistic, especially in 3D images where differences in imaging setups often results in contrast differences and CT/MR-related artifacts such as beam hardening and motion artifacts. Furthermore, the image registration process of LR and HR scans introduces another level of difficulty to the SR task. 
- When simply downsampling the images synthetically, the SR task is a lot easier than upsampling an actual LR scan to a corresponding HR scan with a smaller voxel size. Most model perform very well on downsampled data, making it more difficult to measure performance differences between methods. 
- To enable further model development in volumetric super-resolution and improve generalization across volumetric image domains, we introduce a new \textbf{Vo}lumetric \textbf{Da}taset for \textbf{Su}per-\textbf{Re}solution, \datasetname, featuring a multi-resolution scans of samples from different mircrostructural domains. 


Volumetric super-resolution is an emerging research topic in Computer Vision with a wide range of applications. Compared with 2D SR, volumetric super-resolution  

While super-resolution approaches have experienced substantial advancements recently, the range of 3D datasets commonly used for volumetric super-resolution have extremely narrow applicability. Unlike 3D datasets, 2D datasets are designed to support a wide range 

Specifically, most super-resolution frameworks still rely on synthetic image degradation techniques to establish the LR-HR image pairs to provide training examples. 

As state-of-the-art super-resolution frameworks rely on supervised training where correspondence between the LR and HR image is assumed, degradation techniques are convienient as one does not have to deal with registration.    

We introduce a new \textbf{Vo}lumetric \textbf{Da}taset for \textbf{Su}per-\textbf{Re}solution (\datasetname) featuring a wide range of mircrostructural image domains. 

In recent years, volumetric super-resolution (SR) and related 3D vision tasks have largely been explored through datasets comprised of medical images acquired using Computed Tomography (CT) or Magnetic Resonance Imaging (MRI). 

0) In recent years, volumetric super-resolution (SR) and related 3D vision tasks have largely been explored through datasets comprised of medical images acquired using Computed Tomography (CT) or Magnetic Resonance Imaging (MRI). 

1) Yet, despite the growing  application 

1) Acquiring high-quality volumetric image datasets requires expert knowledge, expensive imaging setups, and is very time consuming. Furthermore, the data is more difficult to preprocesss due to the large volumes of data.

2) Unlike 2D image datasets, which are usually designed for general applicability and often contain a diverse image scenes, volumetric image datasets are highly specialized to address a specific scientific problem, comprising a very narrow range of unique image structures. 


%While medical imaging remains an important area of application for volumetric

Unlike 2D image datasets, which are usually designed for general applicability and often contain a broad range of items and image scenes, volumetric image datasets are highly specialized to address a specific scientific problem, comprising a very narrow range of unique image structures. 

Unlike popular 2D image datasets, volumetric image datasets are highly specialized to address a specific scientific problem, comprising a very narrow range of unique image structures. which are usually designed for general applicability and often contain a broad range of items and image scenes

Due to volumetric image datasets being sparsely available compared with 2D image datasets, volumetric image processing techniques are usually evaluated using a single dataset, as opposed to 2D approaches where datasets are abundant. Because of this combination of small number of available 3D datasets plus methods being evaluated sometimes on a single dataset, it is difficult to benchmark volumetric imaging methods confidently. 




%Deep learning-based volumetric super-resolution methods have shown remarkable advances. These impressive results are, as we will demonstrate, an illusion resulting from the training datasets. The most widely used approach is to use pairs of high and low-resolution volumes, where the corresponding low-resolution volumes are obtained by downsampling the high-resolution volumes \cite{}. The problem is that from real data, i.e., data recorded in both high and low resolution, you get smeared out results -- results that are far from the close-to-perfect predictions obtained from down-sampled data. 

%We have discovered this by experiments carried out on our large-scale CT dataset for super-resolution called \textbf{VoDaSuRe} -- \textbf{Vo}lumetric \textbf{Da}taset for \textbf{Su}per-\textbf{Re}solution. In VoDaSuRe, we have used micro-CT to record samples at different resolutions using the same scanner. To allow comparison to down-sampled data, we also provide a down-sampled version of the data.

%Using VoDaSuRe, we have trained models, either on the scanned low-resolution volumes or on the down-sampled volumes, for predicting high resolution. The models trained on scanned low-resolution differ significantly from the models trained on down-sampled data, as shown in \cref{fig:overview_vodasure}. Models trained on down-sampled data accurately recover structures. But training on data scanned at different resolutions gives predictions with fine structures that are severely smeared out. Surprisingly, predicting from the low-resolution scans, but using models trained on downsampled data, retains a higher level of structure, albeit not nearly as precise as when predicting from the downsampled volumes. These differences in model performance surprised us and must stem from a domain shift from low-resolution scans and down-sampled data. The fact that models perform so differently shows the need for additional research in volumetric super-resolution, now made possible by the VoDaSuRe dataset. 

%The VoDaSuRe volumes vary significantly in their structural regularity and fineness. The scanned samples are different types of wood, wood composites, cardboard, and bone (bovine and human). The bone volumes are relatively simple, since they have high contrast and are smoothly varying, whereas the wood-based samples have coarse to very fine structures, and vary from highly regular solid wood to chaotic composites of wood fibers. 

%Especially, the fine canal structures in wood are lost in low resolution, and models trained on scanned data cannot recover these structures, instead predicting a smeared-out image. However, down-scaled data can recover these structures, even when they disappear in low resolution. The appearance of the smeared-out image is not present in the training data, so the models trained on scanned data shift the distribution of the data from the training data to the predicted data, and this shift is significantly higher for scanned low-resolution data than for down-sampled data.








%In the field of volumetric image processing, method development has largely been explored through datasets of medical images acquired using Computed Tomography (CT) or Magnetic Resonance Imaging (MRI). Unlike 2D image datasets, which are usually designed for general applicability and often contain a broad range of items and image scenes, volumetric image datasets are highly specialized to address a specific scientific problem, comprising a very narrow range of unique image structures. 

%In recent years, volumetric super-resolution (SR) and related 3D vision tasks have largely been explored through datasets comprised of medical images acquired using Computed Tomography (CT) or Magnetic Resonance Imaging (MRI). Unlike 2D image datasets, which are designed to cover a broad range of objects and textures to support general-purpose model development, existing 3D datasets are typically created to address a specific problem, such as segmentation and detection of pathologies. While such datasets are invaluable for clinical research, they represent a narrow range of volumetric structures and contrast variations, limiting their suitability for developing and evaluating generalizable volumetric image processing methods, including volumetric SR approaches.

%Unlike 2D image datasets, which are designed to cover a broad range of objects and textures to support general-purpose model development, existing 3D datasets are typically created to address a specific application, such as segmentation and detection of pathologies. 

%The scarcity of diverse volumetric datasets stems from the inherent challenges of 3D data acquisition. Unlike collection of 2D images, acquiring volumetric images requires complex imaging setups, expert operation, and lengthy acquisition times. Furthermore, each volume consumes significant storage and computational resources, making large-scale data collection and sharing difficult. Consequently, most volumetric image processing methods are evaluated on a small number of datasets, hindering reliable benchmarking and limiting progress toward generalizable models.

%A particular need exists for datasets designed specifically for volumetric super-resolution. In 2D SR research, the availability of large and diverse datasets such as ImageNet, DIV2K, and Flickr2K has driven the development of powerful and broadly applicable models, including recent vision transformer (ViT) architectures. In contrast, volumetric SR remains dominated by medical datasets of brain MRI or clinical CT scans, which offer limited variation in texture, contrast, and structural complexity. Moreover, nearly all existing volumetric SR datasets rely on synthetic degradation model where low-resolution (LR) volumes are generated by downsampling high-resolution (HR) data. While convenient for supervised training, this approach produces overly idealized LR-HR pairs that do not reflect the complexity of real-world acquisition. In practice, low-resolution scans differ from high-resolution ones not only in voxel size, but also in noise characteristics, contrast, and modality-specific artifacts such as beam hardening, motion blur, or partial volume effects. Super-resolving genuinely low-resolution volumetric scans is therefore a substantially harder problem than reconstructing synthetically degraded data. Yet, the lack of co-registered multi-resolution volumetric datasets limits research in this direction. To address this, we introduce the \textbf{Vo}lumetric \textbf{Da}taset for \textbf{Su}per-\textbf{Re}solution (\textbf{VoDaSuRe}), a new benchmark designed specifically for volumetric super-resolution. VoDaSuRe contains real, co-registered multi-resolution scans of samples from diverse microstructural domains, providing a unique platform for evaluating SR methods under realistic imaging conditions. By bridging the gap between synthetic and physically acquired resolution levels, VoDaSuRe enables more robust model development and support for generalization across volumetric image domains. 

\end{comment}

==> sec/2_related_work.tex <==
\section{Related work}
\label{sec:related_work}

\subsection{Super-resolution for volumetric images}
Existing methods for 3D SR can be divided into slice-wise and volumetric approaches; slice-wise SR approaches upscale each image slice independently to increase in-plane resolution. Although computationally efficient, such methods ignore cross-plane information, thereby risking discontinuities across volumetric predictions. Volumetric SR leverages 3D convolutional or ViT layers to learn spatial correlations in all dimensions simultaneously, improving prediction accuracy over slice-wise approaches at the cost of increased computational cost. 

With growing interest in volumetric SR, alternative SR methods have emerged: Axial SR methods have been proposed to increase spatial resolution in the slice direction of low-resolution MRI while preserving in-plane resolution \cite{}. Arbitrary scale SR methods have been proposed to produce continuously upscaled volumetric images using implicit neural representations \cite{}, as well as multi-contrast SR methods that exploit images from multiple imaging modalities to enrich feature extraction and prediction \cite{}. 

Most research in SR methods has been based on data obtained by down-scaling to get LR-HR pairs from the same volume. Unfortunately, this practice simplifies the SR task, as physically acquired low-resolution scans differ fundamentally from downsampled HR data; low-resolution acquisition often enables improved contrast and signal-to-noise ratios, but may introduce acquisition or reconstruction artifacts. To be useful, SR methods must accurately reconstruct high-resolution images despite these artifacts. Therefore, data for developing SR methods must have the same properties as data scanned at different resolutions. Although more sophisticated degradation models have been proposed, progress towards improving the generalization of volumetric SR in real-world scenarios remains limited by the lack of paired multi-resolution volumetric datasets.

\subsection{Volumetric image datasets}
Despite volumetric image datasets varying in acquisition methods, resolution scales, and application domains, medical imaging datasets remain the most commonly used data category for volumetric SR \cite{Ji_3DSR_survey}. The use of SR for medical images is motivated by several factors, enabling increased diagnostic accuracy, improved treatment planning, shorter acquisition times, and alleviated radiation requirements \cite{Chen_mDCSRN_A, Chen_mDCSRN_B, Chen_mDCSRN_C, Ji_3DSR_survey}. 

Several works have studied the enhancement of T1- and T2-weighted structural brain MRI images. The Human Connectome Project (HCP) 1200 subjects release used by \citet{Chen_mDCSRN_A, Chen_mDCSRN_B, Chen_mDCSRN_C}, and others \cite{Lu_novel, Forigua_SuperFormer, li2021volumenet, Wu_ArSSR, zhou2022blind, Wang_MRGD, Hoeg_MTVNet} includes 1113 healthy subjects acquired using a 3T scanner with an isotropic resolution of 0.7 mm. The Information eXtraction from Images (IXI) includes PD-, T1-, and T2-weighted structural MRI from 600 healthy subjects scanned using 3T or 1.5T platforms with a resolution of $0.9375\times0.9375\times1.2$ mm and matrix size of $256\times256\times144\text{-150}$. IXI was used by \citet{li2021volumenet} and others \cite{Zhang_SERAN, Wang_W2AMSN, Huang_TransMRSR, Wang_InverseSR, Li_MFER, Hoeg_MTVNet} for both single- and multi-contrast SR. The Kirby 21 dataset used by \citet{Pham_SRCNN3D} and others \cite{Wang_EDDSR, Zhang_CFTN, Pham_ReCNN, Wang_FASR, Du_DCED, Li_MFER, Hoeg_MTVNet} consists of multi-modality brain MRI from 21 healthy subjects recorded on a 3T platform with a resolution of $1\times0.9375\times0.9375$ mm and a matrix size of $180\times256\times256$. The National Alliance for Medical Image Computing (NAMIC) was used by \cite{iwamoto2022unsupervised, Pham_ReCNN} and includes multi-modality brain MRI of 20 subjects acquired in $1\text{mm}^3$ resolution and $256\times256$ in-plane resolution. \citet{Li_McASSR} studied multi-contrast SR using fastMRI, a large dataset including brain, prostate, breast, and knee MRI acquired with an in-plane resolution of $320\times320$. Pathological brain MRI has also been used; \citet{Pham_SRCNN3D} and others \cite{Wang_EDDSR, Li_McASSR, Zhu_MIASSR, Hoeg_MTVNet} used T2-weighted scans from glioma patients featuring an isotropic resolution of 1 mm and a matrix size of $240\times240\times155$ from the Brain Tumor Segmentation Challenge (BraTS). Brain MRI of Alzheimer patients acquired using 1.5T or 3T at various resolutions from the Alzheimer’s Disease Neuroimaging Initiative (ADNI) was used by \cite{Sanchez_SRGAN3D, Lu_novel}. 

Despite their popularity, these datasets have relatively low resolution, with an in-plane resolution of $\leq 320^2$ voxels. Recent work suggests that the low resolution of current 3D benchmark datasets limits the benefits offered by the larger receptive field of ViTs, preventing proper benchmarking of CNN vs. ViT architectures for volumetric SR \cite{Hoeg_MTVNet}. More recently, higher resolution medical imaging datasets with an in-plane resolution of $512^2$ have emerged, including CTSpine1K \cite{deng_CTSpine1K}, LiTS \cite{bilic_LITS}, KiTS \cite{}, and LIDC-IDRI \cite{Armato_LIDC_IDRI}. Yet, these datasets have not been widely used in volumetric SR.

Due to the complexity of 3D data acquisition, most volumetric datasets provide only a single resolution per scan. To train SR models, low-resolution data are therefore synthetically generated using simple degradation models. Downsampling using a combination of Gaussian smoothing and interpolation, e.g, cubic or linear, is a commonly used practice for the generation of LR-HR paired images for both slice-wise, volumetric, and axial SR approaches. Acknowledging the need to be able to address more complex LR-HR disparities, other degradation methods have been proposed; to simulate the loss in the frequency domain caused by reducing the number of frequency bins of MRI data acquisition, k-space truncation methods have been suggested \cite{Chen_mDCSRN_A, Chen_mDCSRN_B, Chen_mDCSRN_C}. By removing the higher-frequency k-space components of the MRI image, aliasing is introduced in areas of high-frequency spatial variation. This more closely mimics LR MRI data acquisition while preserving the spatial dimensions of the input image. Expanding upon this, \citet{ayaz2024effective} suggested a more comprehensive degradation approach in which they simulate LR data acquisition using a set of tissue relaxation times and MRI sequence parameters, as well as Tukey window filtering and noise addition in the k-space. 

\begin{figure*}[t]
  \includegraphics[width=1.00\linewidth]{figs/VoDaSuRe_preprocessing_4.png}
    \caption{Illustration of our preprocessing pipeline of VoDaSuRe.} 
  \label{fig:VoDaSuRe_preprocessing}
\end{figure*}

\subsection{Paired image datasets for volumetric SR}
Despite advancements in degradation models enabling more realistic generation of LR data from HR images for both 2D and volumetric SR, numerous image degradation factors have yet to be modeled. CT-related artifacts such as beam-hardening, motion, and ring artifacts are difficult to reproduce realistically using synthetic approaches. Because of these effects, the generation of realistic LR data featuring the aforementioned artifacts can still only be done by acquiring paired LR-HR image data of the same sample using different scanning devices or acquisition parameters.

Recognizing this, attempts have been made to construct datasets which realistically capture LR-HR image discrepancies in volumetric data; The Femur Archaeological CT Super-resolution dataset (FACTS) by \citet{bardenfleth2024superresolution} consists of 12 co-registered human femurs scanned using a laboratory micro-CT device and a clinical-CT scanner running a routine hospital scan protocol. Besides decreased resolution, the different scanning devices introduce a notable image domain shift, resulting in a non-trivial volumetric SR task.     

\citet{RPLHR_CT} proposed the RPLHR-CT dataset, which contains 250 paired chest CT volumes from patients. The high- and low-resolution volumes were obtained by reconstructing the CT volumes using a subset of the original slices, producing volumes with the same in-place resolution but increased slice thickness. 

\citet{chu2025paired} curated a multi-model dataset containing 20 paired brain MRI scans acquired using a 3T and a 7T MRI scanning device, enabling unimodal and cross-model SR tasks on real-world data. Low-resolution T2w scans were acquired at 0.9 x 0.9 x 1.0 mm resolution and matrix size of 256 x 256 x 90 voxels, while high-resolution T2w scans were acquired with a resolution of 0.4 x 0.4 x 1.0 mm and matrix size 480 x 512 x 224 voxels. T1w scans as well as hippocampus segmentation labels are also available. 

Similarly, \citet{li2022deep} collected a paired dataset of 20 MRI brain scans where LR volumes were acquired from a variety of 1.5T scanning devices from different hospitals, and corresponding HR volumes were collected with a 3T scanning device operating a research scanning protocol. 

The 2016 Low Dose CT (LDCT) Grand Challenge contains 299 CT scans, of which 200 scans are publicly available. 99 head scans, 100 chest scans, and 100 abdomen scans were acquired using routine dose levels for their respective anatomical region. Each paired scan includes a full dose, and a simulated lower dose level, with head and abdomen provided at 25\% of the routine dose and chest scans provided at 10\% of the routine dose. The reduced dose results in a noticeable decrease in contrast and increased noise, providing a unique image restoration task.

Within the field of synchrotron CT imaging, \citet{green2025three} presented the I13-2 XCT dataset, a multi-modal CT imaging dataset featuring a Zinc-Doped Zeolite 13X sample, a material commonly used in the carbon capture industry, scanned at 4 four pixel-sizes: 2.6 um, 1.625 um, 0.8125 um and 0.325 um. The volumes feature a size 2510 x 2510 x 2110 for each resolution, producing a set of large-scale SR tasks across multiple imaging scales. 

\citet{solidbattery2023} applied a Residual Encoder-Decoder Network (RED-Net) on a paired set of Lab-CT and synchrotron CT scans of an all-solid-state battery cathode to mimic the increased contrast enabled by a synchrotron x-ray source. 

In \cite{synchrotronfiber2023}, synchrotron data in two resolutions were acquired of a fiber composite material by changing the microscope magnification of the detector. A super-resolution GAN was trained to perform 4x upsampling of the LR volume. They acquired 1 LR and 1 HR volume, as well as 17 LR validation volumes.

\citet{mcnabb2025wand} proposed WAND, a large volumetric dataset featuring brain MRI from 170 patients recorded using several imaging devices across a wide range of modalities and scanning protocols. 

Very recently, \citet{klos2025super} applied quantification of SR-enhanced volumes to quantify the characteristics of pores and defects in lattice structures. The authors created a multi-resolution volumetric dataset by scanning a diamond-like lattice cuboid sample using a Lab-CT device in six isotropic resolutions ranging from 3um to 18um.  

Although these works push the boundary and enable more realistic SR tasks, the volumes within these datasets are either 1) small-scale volumes ($\leq 512^3$), 2) span a narrow set of microstructure image domains, 3) offer a small number of volumes in total, 4) or are not easy to download. Their limited size and narrow domain coverage prevent fair and reproducible comparison between methods. In contrast, VoDaSuRe provides registered, real multi-resolution volumetric scans acquired across multiple microstructural domains, offering the first large-scale benchmark for studying genuine resolution enhancement in volumetric imaging.

\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.1}

% ---- First table ----
\resizebox{\textwidth}{!}{%
\begin{NiceTabular}{cccccccccccccccc}[hvlines]
\Block{2-1}{Method}
& \Block{2-1}{CTSpine1K} 
& \Block{2-1}{LiTS} 
& \Block{2-1}{LIDC-IDRI} 
& \Block{2-1}{VoDaSuRe \\(Downsampled)} 
& \Block{2-1}{VoDaSuRe \\(Registered)} \\
\\
Scale $2\times$ 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE}
& \footnotesize{PSNR / SSIM / NRMSE} \\ \hline\hline

HAT & 35.94 / .9258 / .0430 & 38.11 / .9713 / .0339 & 33.92 / .9062 / .0418 & 23.32 / .8921 / .1638 &  17.44 / .4755 / .3377 \\ 
RCAN & 36.62 / .9282 / .0402 & 39.04 / .9736 / .0309 & 35.01 / .9111 / .0378 & 23.28 / .8687 / .1654 & 17.40 / .4691 / .3337 \\ 
EDDSR & 36.82 / .9244 / .0388 & 39.53 / .9694 / .0284 & 34.17 / .9010 / .0403 & 24.86 / .9066 / .1445 & 17.63 / .4755 / .3277 \\ 
SuperFormer & 38.33 / .9328 / .0337 & 41.53 / .9780 / .0228 & 37.18 / .9161 / .0309 & 25.00 / .9090 / .1429 & 18.17 / .5246 / .3089 \\ 
MFER & 39.06 / .9324 / .0317 & 43.15 / .9774 / .0194 & 38.83 / .9158 / .0274 & 25.30 / .9093 / .1404 &  17.98 / .5152 / .3184 \\ 
mDCSRN & 38.88 / .9352 / .0317 & 42.58 / .9798 / .0203 & 37.83 / .9190 / .0290 & 25.17 / .9089 / .1438 & 17.97 / .5110 / .3149 \\ 
MTVNet & 39.31 / .9354 / .0306 & 43.26 / .9801 / .0191 & 39.54 / .9214 / .0259 & 24.82 / .9066 / .1479 & 18.21 / .5249 / .3080 \\  
RRDBNet3D & 39.88 / .9387 / .0288 & 44.81 / .9821 / .0161 & 40.47 / .9256 / .0239 & 25.50 / .9106 / .1397 & 18.25 / .5377 / .3057 \\ 
\end{NiceTabular}
}

\vspace{0.1cm}

% ---- Second table ----
\resizebox{\textwidth}{!}{%
\begin{NiceTabular}{cccccccccccccccc}[hvlines]
\Block{2-1}{Method}
& \Block{2-1}{CTSpine1K} 
& \Block{2-1}{LiTS} 
& \Block{2-1}{LIDC-IDRI} 
& \Block{2-1}{VoDaSuRe \\(Downsampled)} 
& \Block{2-1}{VoDaSuRe \\(Registered)} \\
\\
Scale $4\times$ 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE}
& \footnotesize{PSNR / SSIM / NRMSE} \\ \hline\hline

HAT & 30.42 / .8391 / .0841 & 31.71 / .9106 / .0733 & 29.49 / .8270 / .0723 &  16.61 / .5032 / .3553 & 15.41 / .3543 / .4526 \\ 
RCAN & 31.38 / .8511 / .0758 & 32.82 / .9229 / .0653 & 30.71 / .8416 / .0635 & 16.95 / .5512 / .3434 & 15.37 / .3235 / .4146 \\ 
EDDSR & 31.51 / .8483 / .0732 & 33.10 / .9205 / .0616 & 30.04 / .8351 / .0680 & 18.15 / .6222 / .3051 & 15.82 / .3995 / .3889 \\ 
SuperFormer & 33.95 / .8674 / .0561 & 35.58 / .9396 / .0457 & 33.23 / .8616 / .0476 &  18.53 / .6415 / .2931 & 16.24 / .4395 / .3729 \\ 
MFER & 34.35 / .8720 / .0540 & 36.17 / .9439 / .0447 & 33.40 / .8658 / .0527 &  18.58 / .6518 / .2898 & 15.99 / .4187 / .3851 \\ 
mDCSRN & 34.78 / .8741 / .0512 & 36.57 / .9461 / .0407 & 33.93 / .8689 / .0437 &  18.65 / .6666 / .2871 &  16.11 / .4257 / .3808 \\ 
MTVNet & 34.39 / .8742 / .0539 & 36.25 / .9464 / .0428 & 33.76 / .8696 / .0452 &  18.81 / .6619 / .2888 & 16.18 / .4204 / .3775 \\ 
RRDBNet3D & 35.57 / .8803 / .0472 & 37.86 / .9526 / .0353 & 35.26 / .8761 / .0387 &  19.08 / .6779 / .2746 & 16.22 / .4390 / .3729 \\ 
\end{NiceTabular}
}

\caption{Quantitative comparison of state-of-the-art SR models on datasets CTSpine1K, LiTs, LIDC-IDRI and \datasetname using downsampled and registered LR input data. The best and second best metrics PSNR $\uparrow$ / SSIM $\uparrow$ / NRMSE $\downarrow$ are highligthed in \textcolor{red}{red} and \textcolor{blue}{blue}.}
\vspace{-0.05in}
\label{tab:table_quantitative_results_in_domain}
\end{table*}


\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.1}

% ---- Second table ----
\resizebox{\linewidth}{!}{%
\begin{NiceTabular}{ccccc}[hvlines]
\Block{1-1}{Training} & \Block{1-1}{\footnotesize{VoDaSuRe (Registered)}} & \Block{1-1}{\footnotesize{VoDaSuRe (Downsampled)}} \\
\Block{1-1}{Evaluation} & \Block{1-1}{\footnotesize{VoDaSuRe (Downsampled)}} & \Block{1-1}{\footnotesize{VoDaSuRe (Registered)}} \\

Scale $4\times$ & \footnotesize{PSNR / SSIM / NRMSE} & \footnotesize{PSNR / SSIM / NRMSE} \\ \hline\hline
HAT & 14.93 / .2842 / .5219 & 14.58 / .3118 / .4445 \\
MFER & 14.85 / .3279 / .4467 & 14.89 / .3837 / .4296 \\
RCAN & 14.91 / .2366 / .4597 & 14.57 / .3429 / .4433 \\
MTVNet & 15.39 / .3447 / .4183 & 14.72 / .3540 / 0.4407 \\
RRDBNet3D & 15.51 / .3838 / .4051 & 14.94 / .3923 / .4221 \\
mDCSRN & 15.81 / .4198 / .4013 & 14.94 / .4000 / 0.4266 \\
EDDSR & 16.02 / .4238 / .3819 & 15.18 / .3945 / .4202 \\
SuperFormer & 16.05 / .4411 / 0.3964 & 15.12 / .3895 / .4191 \\

\end{NiceTabular}
}

\caption{Quantitative results for cross-domain experiments on \datasetname registered and downsampled at scale $4\times$.}
\vspace{-0.05in}
\label{tab:cross_domain_experiments}
\end{table}














\begin{comment}

# Comments

Hvilke dataset bruges til volumetrisk SR?
Hvilke degradation metoder bruges til at simulere low-resolution input data?
Hvilke strukturelle domæner indgår typisk i de dataset der findes?


Hvilke parrede dataset findes til volumetrics super-resolution?
Hvordan er fordeling af antal volumener, volumenernes størrelse, og totale antal voxels i andre parrede 3D dataset?
Hvilke strukturelle domæner dækker disse dataset?

# Notes

    - Degradation models for 2D and 3D super-resolution
        - Downsampling (2D)
        - More "real-world" SR (Downsampling, JPEG compression, gaussian noise, etc.) (2D)
        - Slice-removal (3D)
        - K-space truncation (only for 3D)

    - Paired datasets for volumetric SR
        - 

    - Large-scale datasets for volumetric SR

    - Next-generation data formats
    
\end{comment}

%\subsection{Super-resolution for volumetric images}

\begin{comment}

	- Volumetric super-resolution
		○ What is volumetric SR?
		○ What is the motivation?
		○ What different approaches exists for volumetric SR, such as slice-wise, axial, and multi-modal approaches?
		○ Which notable methods exist?
        ○ Progress in volumetric SR is limited by: 
        1) Degradation methods that do not correspond well to real-world multi-resolution scans, and the lack of multi-resolution datasets. 
        2) Lack of datasets that cover a broad range of microstructures (models are benchmarked on datasets featuring a narrow set of image structures, making fair architectural comparisons difficult).
        3) Low resolution datasets: models are benchmarked on datasets consisting of low-resolution volumes. Mention MTVNet paper here, and that performance may depend on resolution.

\end{comment}

\begin{comment}

%Super-resolution (SR) in volumetric image aims to recover high-resolution (HR) 3D structures from low-resolution (LR) input volumes. %The use of SR for volumetric images has widespread application in medical and scientific imaging, allowing finer microstructural analysis while enabling reduced scan time and radiation exposure without the need for hardware replacement. 
Existing methods for 3D SR can be divided into slice-wise and volumetric approaches; slice-wise SR approaches upscale each image slice independently to increase in-plane resolution. Although computationally efficient, such methods ignore cross-plane information, thereby risking discontinuities across volumetric predictions. Volumetric SR leverages 3D convolutional or ViT layers to learn spatial correlations in all dimensions simultaneously, improving prediction accuracy over slice-wise approaches at the cost of increased computational cost. 

With growing interest in volumetric SR, alternative SR methods have emerged: Axial SR methods have been proposed to increase spatial resolution in the slice direction of low-resolution MRI while preserving in-plane resolution \cite{}. Arbitrary scale SR methods have been proposed to produce continuously upscaled volumetric images using implicit neural representations \cite{}, as well as multi-contrast SR methods that exploit images from multiple imaging modalities to enrich feature extraction and prediction \cite{}. 

Most research in SR methods has been based on data obtained by down-scaling to get LR-HR pairs from the same volume. Unfortunately, this practice simplifies the SR task, as physically acquired low-resolution scans differ fundamentally from downsampled HR data; low-resolution acquisition often enables improved contrast and signal-to-noise ratios, but may introduce acquisition or reconstruction artifacts. To be useful, SR methods must accurately reconstruct high-resolution images despite these artifacts. Therefore, data for developing SR methods must have the same properties as data scanned at different resolutions. Although more sophisticated degradation models have been proposed, progress towards improving the generalization of volumetric SR in real-world scenarios remains limited by the lack of paired multi-resolution volumetric datasets.
\end{comment}

\begin{comment}

Implicit Neural Representation 

, axial SR approaches leverage cross-plane modeling to increase spatial resolution in the slice direction while preserving in-plane resolution. %\citet{} developed an axial SR is typically used to reduce slice thickness in low-resolution MRI acquisition.

Lastly, multi-contrast SR approaches exploit images from multiple imaging modalities to enrich feature extraction


%In a compromise to reduce scan time in clinical settings, medical images are usually with a slice thickness greater than the in-plane resolution. To address this, axial SR approaches have been developed to increase spatial resolution in the slice direction while preserving in-plane resolution. Lastly, multi-contrast SR approaches exploit images from multiple imaging modalities to enrich feature extraction...  

\end{comment}


%\subsection{Volumetric image datasets}

\begin{comment}
	- Volumetric datasets
		○ Which datasets are commonly used for volumetric SR and 3D deep learning?
		○ Which domains do they occupy?
		○ Which degradation methods are used for volumetric SR?
		○ Which data formats do they use?

Volumetric dataset are Low-resolution...

Additionally, existing volumetric datasets are stored in formats like NIfTI, DICOM, or Zarr, each optimized for specific imaging pipelines but rarely standardized across datasets. This fragmentation, combined with the scarcity of publicly available 3D data, has limited consistent benchmarking in volumetric SR.

\end{comment}

\begin{comment}
\begin{itemize}
    \item Downsampling (2D)
    \item More "real-world" SR (Downsampling, JPEG compression, gaussian noise, etc.) (2D)
    \item Slice-removal (3D)
    \item K-space truncation (only for 3D)
    \item Specialized LR MRI degradation methods \citet{ayaz2024effective} 
\end{itemize}    
\end{comment}


\begin{comment}
Sui et al. [149] designed an MR image degrada-
tion model by estimating blur kernels from the data.
Moreover, Zhou et al. [67] proposed the blind super-reso-
lution approach in an unsupervised manner. Initially, they
employ a CycleGAN-based architecture to generate low-
resolution images, achieving the domain correction. Sub-
sequently, they use the upscaling network that was trained
using HR-LR pairs to facilitate accurate reconstruction.
Furthermore, Iwamoto et al. [65] also proposed an unsu-
pervised multi-contrast MR image super-resolution
method. Thus more effective real MR image super-reso-
lution approaches benefitted the clinical application are
urgently studied.    



Volumetric image datasets span a variety of acquisition methods including Laboratory CT, synchrotron imaging, and medical imaging techniques such as MR and CT. Volumetric datasets are typically acquired with a specific analysis goal in mind, and usually contain a small set of sample instances of a particular structure of interest. 

Volumetric datasets used in SR and related 3D vision tasks are typically derived from medical imaging domains. Common examples include BraTS for brain tumor segmentation, LiTS for liver lesion analysis, KiTS for kidney tumor segmentation, and FastMRI for brain, knee and prostate. These datasets have been instrumental for supervised learning in clinical contexts but represent narrow imaging domains with limited variation in structural content and modality diversity.

With advancements in MR imaging enabling near risk-free data collection of human anatomy, initiatives have been made to collect and curate standardized volumetric datasets of human organs.  General brain MRI datasets include the IXI dataset, the Human Connectome Project (HCP 1200) and the Kirby 21 dataset. FastMRI contains brain MRI, knee and prostate images. 

Due to the high cost and complexity of 3D data acquisition, most volumetric datasets provide only a single resolution per scan. To train SR models, low-resolution data are therefore synthetically generated using simple degradation models such as Gaussian blur and uniform downsampling. 

Downsampling using a combination of smoothing and some image interpolation function (nearest-neighbour, linear, etc.) remains by far the most commonly used practice for generation of LR-HR paired images for super-resolution. 

Acknowledging the need to be able to address more complex LR-HR disparities, \citet{} proposed a degradation scheme using a combination of downsampling, gaussian noise, compression artifacts, and more to increase the versatility of SR approaches on 2D images.

To simulate the loss in the frequency domain caused by reducing the number of frequency bins of MRI data acquisition, k-space truncation methods can have been suggested. By removing the higher-frequency k-space components of the MRI image, aliasing is introduced in areas of high-frequency spatial variation. This more close mimics LR MRI data acquisition while preserving the spatial dimensions of the input image.

Expanding upon this, \citet{ayaz2024effective} suggested a more comprehensive degradation approach in which they simulate LR data acquisition using a set of tissue relaxation times and MRI sequence parameters, as well as Tukey window filtering and noise addition in the k-space. 

While convenient, such degradations overlook the complex physics of 3D imaging systems. 

- 3D datasets for deep learning are scarse compared with 2D datasets due to the complicated acquisition process. 
- The datasets used for volumetric SR and related 3D vision tasks are medical imaging datasets. 
- the 3D datasets have low resolution, usually less than 512 along any plane.  Yet, Increasing resolution beyond this is difficult both acquisitionally and practically. medical imaging devices are usually low resolution. Also, with increased resolution the and data size grows quickly and becomes difficult to handle computationally, and sharing becomes. Medical data is also sensitive, further limiting sharing of data.
- 3D datasets are fundamentally different from 2D datasets in that they usually attempt to adresss a specific scientific question, and usually contain images only of a specific organ or pathology. In contrast, 2D datasets are designed for general applicability in mind, and feature scenes with largely varying semantic compositions. The lack of image variety seen in commonly used 3D datasets limits generalizability, and makes fair performance evaluation difficult. 



Despite volumetric imaging datasets varying in acquisition methods, resolution scales and application domains, medical imaging datasets remains the most commonly used data category for volumetric SR, and other related 3D visions tasks such as segmentation, classification and detection. Advances in medical imaging techniques have increased availability of volumetric images, and their analysis is greatly motivated by their scientific impact for improving diagnosis and treatment planning within specific application domains. In brain structural brain MRI, datasets such as Information eXtraction from Images (IXI) 

In structural brain MRI, Information eXtraction from Images (IXI), Human Connectome Project, Kirby 21 and fastMRI. 
CTSpine1K
LiTS
KiTS
LIDC-IDRI

Despite volumetric imaging datasets varying in acquisition methods, resolution scales and application domains, medical imaging datasets remains the most commonly used data category for volumetric SR. Advances in medical imaging techniques have increased the availability of volumetric images, and their analysis is greatly motivated by their scientific impact for improving diagnosis and treatment planning within specific application domain. Several works have studied enhancement structural brain MRI images;  
\citet{Chen_mDCSRN_A, Chen_mDCSRN_B, Chen_mDCSRN_C}. \citet{Forigua_SuperFormer} and others \cite{Lu_novel} (MRGD, 3D FSRCNN, VolumeNet) used structural MRI from Human Connectome Project (HCP)

Kirby 21:
To explore the ability to reconstruct HR volume for realistic
typical anatomical brain structures, we applied the recon-
struction algorithms on T1-weighted MRI images of the
Kirby 21 (twenty-one healthy volunteers with no history of
neurological conditions) [8]. These MPRAGE data were ac-
quired using a 3-T MR scanner (Achieva, Philips Healthcare,
Best, The Netherlands) with a 1.0×1.0×1.2 mm3 resolution
over an FOV of 240 × 204 × 256 mm acquired in the sagittal
plane. 10 images were used for training the neural network
(i.e. from 33th to 42th images) and 5 other images for testing
(i.e. from 1st to 5th images). As in [9], LR images have been
generated by using a Gaussian blur with standard deviation
σ = 1 before a down-sampling by isotropic scale factor 2.

%with commonly used datasets including the Alzheimer’s Disease Neuroimaging Initiative (ADNI), Information eXtraction from Images (IXI), Human Connectome Project (HCP), Kirby 21, the National Alliance for Medical Image Computing (NAMIC) and the Brain Tumor Segmentation Challenge (BraTS). 

%Several works have used \citet{} brain and knee images from the fastMRI.  

First try:
Despite volumetric image datasets varying in acquisition methods, resolution scales and application domains, medical imaging datasets remains the most commonly used data category for volumetric SR \cite{Ji_3DSR_survey}. Enhancement of medical images using is motivated by several factors, including increased diagnostic accuracy, improved treatment planning, shorter acquisition times, and alleviated radiation requirements \cite{Chen_mDCSRN_A, Chen_mDCSRN_B, Chen_mDCSRN_C, Ji_3DSR_survey}. Several works have studied enhancement of T1- and T2-weighted structural brain MRI; \citet{Pham_SRCNN3D} and others \cite{Wang_EDDSR, Zhang_CFTN, Pham_ReCNN, Wang_FASR, Du_DCED, Li_MFER} used the Kirby 21 dataset, which includes 21 healthy scans in $1.0 \times1.0\times1.2$ $\text{mm}^3$ resolution. Brain MRI images from the Alzheimer’s Disease Neuroimaging Initiative (ADNI)  was used by \cite{Sanchez_SRGAN3D, Lu_novel}. \citet{li2021volumenet}. \cite{Zhang_SERAN, Wang_W2AMSN, Huang_TransMRSR, Wang_InverseSR, Li_MFER} used brain MRI images from Information eXtraction from Images (IXI). \citet{Chen_mDCSRN_A, Chen_mDCSRN_B, Chen_mDCSRN_C}, and others \cite{Lu_novel, Forigua_SuperFormer, li2021volumenet, Wu_ArSSR, zhou2022blind, Wang_MRGD} used T1-weighted brain MRI images from the Human Connectome Project (HCP) 1200 subjects release dataset. \citet{Li_McASSR} used brain and knee images from the fastMRI dataset. The National Alliance for Medical Image Computing (NAMIC) was used by \cite{Wang_EDDSR, iwamoto2022unsupervised, Pham_ReCNN}. The Brain Tumor Segmentation Challenge (BraTS) was used by \cite{Pham_SRCNN3D, Li_McASSR, Zhu_MIASSR}.

Despite their popularity these datasets are relatively low-resolution in-plane resolution of approx $\leq 320^2$. Recent work suggests that the low-resolution of current 3D benchmark datasets are limiting the benefits offered by the larger receptive field of ViTs, preventing proper benchmarking of CNN vs. ViT architectures for volumetric SR \cite{Hoeg_MTVNet}.

More recently, higher resolution medical imaging datasets with an in-plane resolution of $512^2$ have emerged, including CTSpine1K, LiTS, KiTS and 
LIDC-IDRI. However, these datasets yet to see widespread usage within volumetric SR. %These feature an in-plane resolution of $512^2$, yet this is still small compared with 2D image datasets which often feature resolutions of $\geq 1000$ in height and width. 

Due to the complexity of 3D data acquisition, most volumetric datasets provide only a single resolution per scan. To train SR models, low-resolution data are therefore synthetically generated using simple degradation models such as Gaussian blur and uniform downsampling. 

Downsampling using a combination of smoothing and some image interpolation function (nearest-neighbour, linear, etc.) remains by far the most commonly used practice for generation of LR-HR paired images for super-resolution. 

%Volumetric image datasets span a variety of acquisition methods including laboratory CT, synchrotron imaging, and medical imaging techniques. The datasets used in volumetric SR are predominantly derived from medical imaging domains such as MR and CT. 

%Other 3D vision tasks including segmentation, classification and detection. 



\end{comment}

\begin{comment}
Despite volumetric image datasets varying in acquisition methods, resolution scales, and application domains, medical imaging datasets remain the most commonly used data category for volumetric SR \cite{Ji_3DSR_survey}. The use of SR for medical images is motivated by several factors, enabling increased diagnostic accuracy, improved treatment planning, shorter acquisition times, and alleviated radiation requirements \cite{Chen_mDCSRN_A, Chen_mDCSRN_B, Chen_mDCSRN_C, Ji_3DSR_survey}. 

Several works have studied enhancement of T1- and T2-weighted structural brain MRI images. The Human Connectome Project (HCP) 1200 subjects release used by \citet{Chen_mDCSRN_A, Chen_mDCSRN_B, Chen_mDCSRN_C}, and others \cite{Lu_novel, Forigua_SuperFormer, li2021volumenet, Wu_ArSSR, zhou2022blind, Wang_MRGD, Hoeg_MTVNet}  includes 1113 healthy subjects acquired using a 3T scanning with an isotropic resolution of 0.7 mm. The Information eXtraction from Images (IXI) includes PD-, T1-, and T2-weighted structural MRI from 600 healthy subjects scanned using 3T or 1.5T platforms with a resolution of $0.9375\times0.9375\times1.2$ mm and matrix size of $256\times256\times144\text{-150}$. IXI was used by \citet{li2021volumenet} and others \cite{Zhang_SERAN, Wang_W2AMSN, Huang_TransMRSR, Wang_InverseSR, Li_MFER, Hoeg_MTVNet} for both single- and multi-contrast SR. The Kirby 21 dataset used by \citet{Pham_SRCNN3D} and others \cite{Wang_EDDSR, Zhang_CFTN, Pham_ReCNN, Wang_FASR, Du_DCED, Li_MFER, Hoeg_MTVNet} consists of multi-modality brain MRI from 21 healthy subjects recorded on a 3T platform with a resolution of $1\times0.9375\times0.9375$ mm and a matrix size of $180\times256\times256$. The National Alliance for Medical Image Computing (NAMIC) was used by \cite{iwamoto2022unsupervised, Pham_ReCNN} and includes multi-modality brain MRI of 20 subjects acquired in $1\text{mm}^3$ resolution and $256\times256$ in-plane resolution. \citet{Li_McASSR} studied multi-contrast SR using fastMRI, a large dataset including brain, prostate, breast and knee MRI acquired with an in-plane resolution of $320\times320$. Pathological brain MRI has also been used; \citet{Pham_SRCNN3D} and others \cite{Wang_EDDSR, Li_McASSR, Zhu_MIASSR, Hoeg_MTVNet} used T2-weighted scans from glioma patients featuring an isotropic resolution of 1 mm and a matrix size of $240\times240\times155$ from the Brain Tumor Segmentation Challenge (BraTS). Brain MRI of Alzheimer patients acquired using 1.5T or 3T at various resolutions from the Alzheimer’s Disease Neuroimaging Initiative (ADNI) was used by \cite{Sanchez_SRGAN3D, Lu_novel}. 

Despite their popularity these datasets are relatively low-resolution with an in-plane resolution of $\leq 320^2$ voxels. Recent work suggests that the low-resolution of current 3D benchmark datasets limits the benefits offered by the larger receptive field of ViTs, preventing proper benchmarking of CNN vs. ViT architectures for volumetric SR \cite{Hoeg_MTVNet}. More recently, higher resolution medical imaging datasets with an in-plane resolution of $512^2$ have emerged, including CTSpine1K \cite{deng_CTSpine1K}, LiTS \cite{bilic_LITS}, KiTS \cite{}, and LIDC-IDRI \cite{Armato_LIDC_IDRI}. Yet, these datasets have not seen widespread usage within volumetric SR. %These feature an in-plane resolution of $512^2$, yet this is still small compared with 2D image datasets which often feature resolutions of $\geq 1000$ in height and width. 

Due to the complexity of 3D data acquisition, most volumetric datasets provide only a single resolution per scan. To train SR models, low-resolution data are therefore synthetically generated using simple degradation models. Downsampling using a combination of Gaussian smoothing and interpolation, e.g, cubic or linear, is a commonly used practice for the generation of LR-HR paired images for both slice-wise, volumetric, and axial SR approaches. Acknowledging the need to be able to address more complex LR-HR disparities, other degradation methods have been proposed; to simulate the loss in the frequency domain caused by reducing the number of frequency bins of MRI data acquisition, k-space truncation methods have been suggested \cite{Chen_mDCSRN_A, Chen_mDCSRN_B, Chen_mDCSRN_C}. By removing the higher-frequency k-space components of the MRI image, aliasing is introduced in areas of high-frequency spatial variation. This more closely mimics LR MRI data acquisition while preserving the spatial dimensions of the input image. Expanding upon this, \citet{ayaz2024effective} suggested a more comprehensive degradation approach in which they simulate LR data acquisition using a set of tissue relaxation times and MRI sequence parameters, as well as Tukey window filtering and noise addition in the k-space. 

\begin{figure*}[t]
  \includegraphics[width=1.00\linewidth]{figs/VoDaSuRe_preprocessing_4.png}
    \caption{Illustration of our preprocessing pipeline of VoDaSuRe.} 
  \label{fig:VoDaSuRe_preprocessing}
\end{figure*}

%While convenient, such degradations overlook the complex physics of 3D imaging systems. 

%Volumetric image datasets span a variety of acquisition methods including laboratory CT, synchrotron imaging, and medical imaging techniques. The datasets used in volumetric SR are predominantly derived from medical imaging domains such as MR and CT. 

%Other 3D vision tasks including segmentation, classification and detection. 

\subsection{Paired image datasets for volumetric SR}

\end{comment}


\begin{comment}

	- Paired datasets for volumetric SR
		○ What datasets exist?
		○ What problem do they serve to solve?
		○ What is the availability of them?
		○ How big are they?

\end{comment}
\begin{comment}
Despite advancements in degradation models enabling more realistic generation of LR data from HR images for both 2D and volumetric SR, numerous image degradation factors have yet to be modeled. CT-related artifacts such as beam-hardening, motion- and ring artifacts are difficult to reproduce realistically using synthetic approaches. %Furthermore, the image registration process required for supervised SR approaches incurs discrepancy between LR-HR data which can be difficult to model, especially if the sample has sustained radiation damage in between scan acquisitions. 
Because of these effects, generation of realistic LR data featuring aforementioned artifacts can still only be done by acquiring paired LR-HR image data of the same sample using different scanning devices or acquisition parameters.

Recognizing this, attempts have been made to construct datasets which realistically capture LR-HR image discrepancies in volumetric data; The Femur Archaeological CT Super-resolution dataset (FACTS) by \citet{bardenfleth2024superresolution} consists of 12 co-registered human femurs scanned using a laboratory micro-CT device and a clinical-CT scanner running a routine hospital scan protocol. Besides decreased resolution, the different scanning devices introduces a notable image domain-shift resulting in a non-trivial volumetric SR task.     

\citet{RPLHR_CT} proposed the RPLHR-CT dataset, which contains 250 paired chest CT volumes from patients. The high- and low-resolution volumes were obtained by reconstructing the CT volumes using a subset of the original slices, producing volumes with the same in-place resolution but increased slice thickness. 

\citet{chu2025paired} curated a multi-model dataset containing 20 paired brain MRI scans acquired using a 3T and a 7T MRI scanning device, enabling unimodal and cross-model SR tasks on real-world data. Low-resolution T2w scans were acquired at 0.9 x 0.9 x 1.0 mm resolution and matrix size of 256 x 256 x 90 voxels, while high-resolution T2w scans where acquired with a resolution of 0.4 x 0.4 x 1.0 mm and matrix size 480 x 512 x 224 voxels. T1w scans as well as hippocampus segmentation labels are also available. 

Similarly, \citet{li2022deep} collected a paired dataset of 20 MRI brain scans where LR volumes were acquired from a variety of 1.5T scanning devices from different hospitals, and corresponding HR volumes were collected with a 3T scanning device operating a research scanning protocol. 

The 2016 Low Dose CT (LDCT) Grand Challenge contains 299 CT scans, of which 200 scans are publicly available. 99 head scans, 100 chest scans and 100 abdomen scans were acquired using routine dose levels for their respective anatomical region. Each paired scan includes a full dose, and a simulated lower dose level, with head and abdomen provided at 25\% of the routine dose and chest scans provided at 10\% of the routine dose. The reduced dose results in a noticeable decrease in contrast and increased noise, providing a unique image restoration task.

Within the field of synchrotron CT imaging, \citet{green2025three} presented the I13-2 XCT dataset, a multi-modal CT imaging dataset featuring a Zinc-Doped Zeolite 13X sample, a material commonly used in the carbon capture industry, scanned at 4 four pixel-sizes: 2.6 um, 1.625 um, 0.8125 um and 0.325 um. The volumes feature a size 2510 x 2510 x 2110 for each resolution, producing a set of large-scale SR tasks across multiple imaging scales. 

\citet{solidbattery2023} applied a Residual Encoder-Decoder Network (RED-Net) on a paired set of Lab-CT and synchrotron CT scans of an all-solid-state battery cathode to mimic the increased contrast enabled by a synchrotron x-ray source. 

In \cite{synchrotronfiber2023}, synchrotron data in two resolutions were acquired of a fiber composite material by changing the microscope magnification of the detector. A super-resolution GAN was trained to perform 4x upsampling of the LR volume. They acquired 1 LR and 1 HR volume, as well as 17 LR validation volumes.

\citet{mcnabb2025wand} proposed WAND, a large volumetric dataset featuring brain MRI from 170 patients recorded using several imaging devices across a wide range of modalities and scaning protocols. 

Very recently, \citet{klos2025super} applied quantification of SR enhanced volumes in order to quantify the characteristics of pores and defects in lattice structures. The authors created a multi-resolution volumetric dataset by scanning a diamond-like lattice cuboid sample using a Lab-CT device in six isotropic resolutions ranging from 3um to 18um.  

Although these works push the boundary and enable more realistic SR tasks, the volumes within these datasets are either 1) small scale volumes ($\leq 512^3$), 2) span a narrow set of microstructure image domains, 3) offer a small number of volumes in total, 4) or are not publicly available. Their limited size and narrow domain coverage prevent fair and reproducible comparison between methods. In contrast, VoDaSuRe provides registered, real multi-resolution volumetric scans acquired across multiple microstructural domains, offering the first large-scale benchmark for studying genuine resolution enhancement in volumetric imaging.

\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.1}

% ---- First table ----
\resizebox{\textwidth}{!}{%
\begin{NiceTabular}{cccccccccccccccc}[hvlines]
\Block{2-1}{Method}
& \Block{2-1}{CTSpine1K} 
& \Block{2-1}{LiTS} 
& \Block{2-1}{LIDC-IDRI} 
& \Block{2-1}{VoDaSuRe \\(Downsampled)} 
& \Block{2-1}{VoDaSuRe \\(Registered)} \\
\\
Scale $2\times$ 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE}
& \footnotesize{PSNR / SSIM / NRMSE} \\ \hline\hline

HAT & 35.94 / .9258 / .0430 & 38.11 / .9713 / .0339 & 33.92 / .9062 / .0418 & 23.32 / .8921 / .1638 &  17.44 / .4755 / .3377 \\ 
RCAN & 36.62 / .9282 / .0402 & 39.04 / .9736 / .0309 & 35.01 / .9111 / .0378 & 23.28 / .8687 / .1654 & 17.40 / .4691 / .3337 \\ 
EDDSR & 36.82 / .9244 / .0388 & 39.53 / .9694 / .0284 & 34.17 / .9010 / .0403 & 24.86 / .9066 / .1445 & 17.63 / .4755 / .3277 \\ 
SuperFormer & 38.33 / .9328 / .0337 & 41.53 / .9780 / .0228 & 37.18 / .9161 / .0309 & 25.00 / .9090 / .1429 & 18.17 / .5246 / .3089 \\ 
MFER & 39.06 / .9324 / .0317 & 43.15 / .9774 / .0194 & 38.83 / .9158 / .0274 & 25.30 / .9093 / .1404 &  17.98 / .5152 / .3184 \\ 
mDCSRN & 38.88 / .9352 / .0317 & 42.58 / .9798 / .0203 & 37.83 / .9190 / .0290 & 25.17 / .9089 / .1438 & 17.97 / .5110 / .3149 \\ 
MTVNet & 39.31 / .9354 / .0306 & 43.26 / .9801 / .0191 & 39.54 / .9214 / .0259 & 24.82 / .9066 / .1479 & 18.21 / .5249 / .3080 \\  
RRDBNet3D & 39.88 / .9387 / .0288 & 44.81 / .9821 / .0161 & 40.47 / .9256 / .0239 & 25.50 / .9106 / .1397 & 18.25 / .5377 / .3057 \\ 
\end{NiceTabular}
}

\vspace{0.1cm}

% ---- Second table ----
\resizebox{\textwidth}{!}{%
\begin{NiceTabular}{cccccccccccccccc}[hvlines]
\Block{2-1}{Method}
& \Block{2-1}{CTSpine1K} 
& \Block{2-1}{LiTS} 
& \Block{2-1}{LIDC-IDRI} 
& \Block{2-1}{VoDaSuRe \\(Downsampled)} 
& \Block{2-1}{VoDaSuRe \\(Registered)} \\
\\
Scale $4\times$ 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE}
& \footnotesize{PSNR / SSIM / NRMSE} \\ \hline\hline

HAT & 30.42 / .8391 / .0841 & 31.71 / .9106 / .0733 & 29.49 / .8270 / .0723 &  16.61 / .5032 / .3553 & 15.41 / .3543 / .4526 \\ 
RCAN & 31.38 / .8511 / .0758 & 32.82 / .9229 / .0653 & 30.71 / .8416 / .0635 & 16.95 / .5512 / .3434 & 15.37 / .3235 / .4146 \\ 
EDDSR & 31.51 / .8483 / .0732 & 33.10 / .9205 / .0616 & 30.04 / .8351 / .0680 & 18.15 / .6222 / .3051 & 15.82 / .3995 / .3889 \\ 
SuperFormer & 33.95 / .8674 / .0561 & 35.58 / .9396 / .0457 & 33.23 / .8616 / .0476 &  18.53 / .6415 / .2931 & 16.24 / .4395 / .3729 \\ 
MFER & 34.35 / .8720 / .0540 & 36.17 / .9439 / .0447 & 33.40 / .8658 / .0527 &  18.58 / .6518 / .2898 & 15.99 / .4187 / .3851 \\ 
mDCSRN & 34.78 / .8741 / .0512 & 36.57 / .9461 / .0407 & 33.93 / .8689 / .0437 &  18.65 / .6666 / .2871 &  16.11 / .4257 / .3808 \\ 
MTVNet & 34.39 / .8742 / .0539 & 36.25 / .9464 / .0428 & 33.76 / .8696 / .0452 &  18.81 / .6619 / .2888 & 16.18 / .4204 / .3775 \\ 
RRDBNet3D & 35.57 / .8803 / .0472 & 37.86 / .9526 / .0353 & 35.26 / .8761 / .0387 &  19.08 / .6779 / .2746 & 16.22 / .4390 / .3729 \\ 
\end{NiceTabular}
}

\caption{Quantitative comparison of state-of-the-art SR models on datasets CTSpine1K, LiTs, LIDC-IDRI and \datasetname using downsampled and registered LR input data. The best and second best metrics PSNR $\uparrow$ / SSIM $\uparrow$ / NRMSE $\downarrow$ are highligthed in \textcolor{red}{red} and \textcolor{blue}{blue}.}
\vspace{-0.05in}
\label{tab:table_quantitative_results_in_domain}
\end{table*}


\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.1}

% ---- Second table ----
\resizebox{\linewidth}{!}{%
\begin{NiceTabular}{ccccc}[hvlines]
\Block{1-1}{Training} & \Block{1-1}{\footnotesize{VoDaSuRe (Registered)}} & \Block{1-1}{\footnotesize{VoDaSuRe (Downsampled)}} \\
\Block{1-1}{Evaluation} & \Block{1-1}{\footnotesize{VoDaSuRe (Downsampled)}} & \Block{1-1}{\footnotesize{VoDaSuRe (Registered)}} \\

Scale $4\times$ & \footnotesize{PSNR / SSIM / NRMSE} & \footnotesize{PSNR / SSIM / NRMSE} \\ \hline\hline
HAT & 14.93 / .2842 / .5219 & 14.58 / .3118 / .4445 \\
MFER & 14.85 / .3279 / .4467 & 14.89 / .3837 / .4296 \\
RCAN & 14.91 / .2366 / .4597 & 14.57 / .3429 / .4433 \\
MTVNet & 15.39 / .3447 / .4183 & 14.72 / .3540 / 0.4407 \\
RRDBNet3D & 15.51 / .3838 / .4051 & 14.94 / .3923 / .4221 \\
mDCSRN & 15.81 / .4198 / .4013 & 14.94 / .4000 / 0.4266 \\
EDDSR & 16.02 / .4238 / .3819 & 15.18 / .3945 / .4202 \\
SuperFormer & 16.05 / .4411 / 0.3964 & 15.12 / .3895 / .4191 \\

\end{NiceTabular}
}

\caption{Quantitative results for cross-domain experiments on \datasetname registered and downsampled at scale $4\times$.}
\vspace{-0.05in}
\label{tab:cross_domain_experiments}
\end{table}


\end{comment}

\begin{comment}
RRDBNet3D 2x REG selected wood
PSNR SAMPLE LIST: [16.63475013 15.07866187]
SSIM SAMPLE LIST: [0.64306299 0.3389664 ]
NRMSE SAMPLE LIST: [0.32904507 0.39153129]

Elm: 15.07866187, 0.3389664, 0.39153129
Cypress: 16.63475013, 0.64306299, 0.32904507

RRDBNet3D 2x REG all VoDaSuRe samples
PSNR SAMPLE LIST: [15.9365285  15.2552816  17.37010622 30.14545641 15.69030146 17.87381874
 16.70356375 17.07229701 26.51268394 18.1787475 ]
SSIM SAMPLE LIST: [0.41112258 0.35510242 0.67641256 0.95627551 0.41650115 0.25586695
 0.51496336 0.66952321 0.94140302 0.58348376]
NRMSE SAMPLE LIST: [0.35826055 0.36969434 0.29467375 0.19153086 0.36216093 0.25861177
 0.32283923 0.3196097  0.19780792 0.2737313 ]

Elm: 15.2552816, 0.35510242, 0.36969434
Cypress: 17.07229701, 0.66952321, 0.3196097
 
\end{comment}










\begin{comment}
    
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.1}

% ---- Second table ----
\resizebox{\linewidth}{!}{%
\begin{NiceTabular}{ccccc}[hvlines]
\Block{1-1}{Training} & \Block{1-1}{\footnotesize{VoDaSuRe (Registered)}} & \Block{1-1}{\footnotesize{VoDaSuRe (Downsampled)}} \\
\Block{1-1}{Evaluation} & \Block{1-1}{\footnotesize{VoDaSuRe (Downsampled)}} & \Block{1-1}{\footnotesize{VoDaSuRe (Registered)}} \\

Scale $4\times$ & \footnotesize{PSNR / SSIM / NRMSE} & \footnotesize{PSNR / SSIM / NRMSE} \\ \hline\hline
HAT & 14.93 / .2842 / .5219 & 14.58 / .3118 / .4445 \\
RCAN & 14.91 / .2366 / .4597 & 14.57 / .3429 / .4433 \\
EDDSR & 16.02 / .4238 / .3819 & 15.18 / .3945 / .4202 \\
SuperFormer & 16.05 / .4411 / 0.3964 & 15.12 / .3895 / .4191 \\
MFER & 14.85 / .3279 / .4467 & 14.89 / .3837 / .4296 \\
mDCSRN & 15.81 / .4198 / .4013 & 14.94 / .4000 / 0.4266 \\
MTVNet & 15.39 / .3447 / .4183 & 14.72 / .3540 / 0.4407 \\
RRDBNet3D & 15.51 / .3838 / .4051 & 14.94 / .3923 / .4221 \\


\end{NiceTabular}
}

\caption{Quantitative results for training/evaluation on \datasetname at scale $4\times$.}
\vspace{-0.05in}
\label{tab:cross_domain_experiments}
\end{table}


\end{comment}

==> sec/5_implementation.tex <==
\subsection{Implementation details}
\label{subsec:implementation_details}

\begin{comment}



\end{comment}



==> sec/unused.tex <==

\begin{table*}[t]
\centering
%\resizebox{\columnwidth}{!}{% use this to resize table to width of column

\renewcommand{\arraystretch}{1.0}

\begin{small}
\begin{NiceTabularX}{\textwidth}{XXXXXXXX}[hvlines]
\Block{2-1}{Dataset} & \Block{2-1}{Method} & \Block{1-3}{Scale $\times 4$} & & & \Block{1-3}{Scale $\times 2$} \\
& & \footnotesize{PSNR} & \footnotesize{SSIM} & \footnotesize{NRMSE} & \footnotesize{PSNR} & \footnotesize{SSIM} & \footnotesize{NRMSE} \\ \hline\hline

%& & & & & & & & & & & & & \\
\Block{8-1}{CTSpine1K}

& RCAN & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& HAT & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& EDDSR & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& MFER & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& mDCSRN & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& SuperFormer & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ 

& RRDBNet3D & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ 

& \networkname & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ \hline \hline

\Block{8-1}{LITS}

& RCAN & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& HAT & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& EDDSR & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& MFER & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& mDCSRN & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& SuperFormer & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ 

& RRDBNet3D & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ 

& \networkname & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ \hline \hline

\Block{8-1}{LIDC-IDRI}

& RCAN & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& HAT & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& EDDSR & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& MFER & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& mDCSRN & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& SuperFormer & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ 

& RRDBNet3D & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ 

& \networkname & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ \hline 

\CodeAfter
%\tikz \erase (1-3);
%\TikzEveryCell[empty]{draw}

\end{NiceTabularX}
\end{small}

\vspace{0.15cm}

\begin{small}
\begin{NiceTabularX}{\textwidth}{XXXXXXXX}[hvlines]
\Block{2-1}{Dataset} & \Block{2-1}{Method} & \Block{1-3}{Scale $\times 4$} & & & \Block{1-3}{Scale $\times 2$} \\
& & \footnotesize{PSNR} & \footnotesize{SSIM} & \footnotesize{NRMSE} & \footnotesize{PSNR} & \footnotesize{SSIM} & \footnotesize{NRMSE} \\ \hline\hline

%& & & & & & & & & & & & & \\

\Block{8-1}{VoDaSuRe\\Downscaled}

& RCAN & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& HAT & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& EDDSR & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& MFER & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& mDCSRN & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& SuperFormer & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ 

& RRDBNet3D & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ 

& \networkname & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ \hline \hline


\Block{8-1}{VoDaSuRe\\Registered}

& RCAN & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& HAT & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& EDDSR & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& MFER & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& mDCSRN & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\

& SuperFormer & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ 

& RRDBNet3D & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ 

& \networkname & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ & $00.00 \pm 0.00$ & $.0000 \pm .0000$ & $.0000 \pm .0000$ \\ \hline 

\CodeAfter
%\tikz \erase (1-3);
%\TikzEveryCell[empty]{draw}

\end{NiceTabularX}
\end{small}

\vspace{0.15cm}


%} % use this to resize table to width of column

\caption{A test caption}
\vspace{-0.05in}
\label{tab:table_quantitative_results}
\end{table*}






\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.1}

% ---- Second table ----
\resizebox{\textwidth}{!}{%
\begin{NiceTabular}{cccccccccccc}[hvlines]
\Block{2-1}{Train} 
& \Block{2-1}{Eval} 
& \footnotesize{RCAN} 
& \footnotesize{HAT} 
& \footnotesize{EDDSR} 
& \footnotesize{SuperFormer} 
& \footnotesize{MFER} 
& \footnotesize{mDCSRN} 
& \footnotesize{MTVNet} 
& \footnotesize{RRDBNet3D} \\

& & \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} 
& \footnotesize{PSNR / SSIM / NRMSE} \\

\Block{1-1}{VoDaSuRe}  & \Block{1-1}{VoDaSuRe}  & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\

\end{NiceTabular}
}

\caption{Quantitative results for different datasets at scales $4\times$ and $2\times$.}
\vspace{-0.05in}
\label{tab:templatetest2}
\end{table*}





\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.1}

% ---- Second table ----
\resizebox{\linewidth}{!}{%
\begin{NiceTabular}{cccccccccccc}[hvlines]
\Block{1-1}{Train} 
& \Block{1-1}{Eval} 
& \footnotesize{RCAN} 
& \footnotesize{HAT} 
& \footnotesize{EDDSR} 
& \footnotesize{SuperFormer} 
& \footnotesize{MFER} 
& \footnotesize{mDCSRN} 
& \footnotesize{MTVNet} 
& \footnotesize{RRDBNet3D} \\

VoDaSuRe & VoDaSuRe & 00.00 / .0000 & 00.00 / .0000 & 00.00 / .0000 & 00.00 / .0000 & 00.00 / .0000 & 00.00 / .0000 & 00.00 / .0000 & 00.00 / .0000 \\

\end{NiceTabular}
}

\caption{Quantitative results for different datasets at scales $4\times$ and $2\times$.}
\vspace{-0.05in}
\label{tab:templatetest2}
\end{table}


\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.1}

% ---- Second table ----
\resizebox{\textwidth}{!}{%
\begin{NiceTabular}{cccccccccccc}[hvlines]
\Block{1-1}{Train} 
& \Block{1-1}{Eval} 
& \footnotesize{PSNR / SSIM} 
& \footnotesize{PSNR / SSIM} 
& \footnotesize{PSNR / SSIM} 
& \footnotesize{PSNR / SSIM} 
& \footnotesize{PSNR / SSIM} 
& \footnotesize{PSNR / SSIM} 
& \footnotesize{PSNR / SSIM}  
& \footnotesize{PSNR / SSIM}  \\

VoDaSuRe & VoDaSuRe & 00.00 / .0000 & 00.00 / .0000 & 00.00 / .0000 & 00.00 / .0000 & 00.00 / .0000 & 00.00 / .0000 & 00.00 / .0000 & 00.00 / .0000 \\

\end{NiceTabular}
}

\caption{Quantitative results for different datasets at scales $4\times$ and $2\times$.}
\vspace{-0.05in}
\label{tab:templatetest2}
\end{table*}






\begin{table*}[t]
\renewcommand{\arraystretch}{1.00}

\begin{subtable}[t]{\linewidth}
\centering
\begin{scriptsize}
%\resizebox{\textwidth}{!}{%
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}cccccccc@{}}
\toprule
Dataset & \#samples & \#volumes & Volume shape & Domain & Modalities & Accessibility & Multi-resolution \\ \midrule

\bottomrule
\end{tabular*}
%}%
\end{scriptsize}
\label{tab:ablation_levels}
\end{subtable}

\caption{Overview of image datasets featuring paired volumetric data}
\label{tab:dataset_table}
\end{table*}






\begin{table*}[t]
\renewcommand{\arraystretch}{1.00}

\begin{subtable}[t]{\linewidth}
\centering
\begin{scriptsize}
%\resizebox{\textwidth}{!}{%
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}cccccccc@{}}
\toprule
Dataset & \#samples & \#volumes & Volume shape & Domain & Modalities & Accessibility & Multi-resolution \\ \midrule
% Tilføj no. of pixels in total 
IXI\footnote{\url{https://brain-development.org/ixi-dataset/}} & 600 & 600 & $256\times256\times(144\text{-}150)$ & Brain MRI & T1w, T2w, PD & Public & \xmark \\ 
HCP 1200 \cite{Van_HCP_1200_dataset} & 1113 & 1113 & $320\times320\times256$ & Brain MRI & T1w, T2w & Public & \xmark \\ 
NAMIC \cite{NAMIC_wiki} & 20 & 20 & $256\times256\times176$ & Brain MRI & T1w, T2w, fMRI, DTI & On request & \xmark \\ 
%ADNI & - & - & $-$ & Brain MRI (Alzheimer's) & - & - & \xmark \\ 
fastMRI \cite{zbontar2018fastmri} & 8400 & 8400 & $256\times256\times20$ (mean) & Brain \& knee MRI & T1w, T2w, FLAIR & Public & \xmark \\ 
BraTS 2023 \cite{Baid_BraTS_GLI, Menze_BraTS_GLI, Bakas_BraTS_GLI, Bakas_BraTS2023_GLI_2} & 1470 & 1470 & $240\times240\times155$ & Brain MRI (Tumor) & T1w, T2w & On request & \xmark \\ 
Kirby 21 \cite{Landman_Kirby21_dataset} & 21 & 43 & $256\times256\times180$ & Brain MRI & T2w, FLAIR, DTI & Public & \xmark \\ 
CTSpine1K \cite{deng_CTSpine1K} & 1005 & 1005 & $512\times512\times(349\textbf{-}659)$ & Spine CT & Clinical CT & Public & \xmark \\ 
LiTS \cite{bilic_LITS} & 130 & 130 & $512\times512\times(0\textbf{-}987)$ & Liver CT & Clinical CT & Public & \xmark \\ 
LIDC-IDRI \cite{Armato_LIDC_IDRI} & 1010 & 1010 & $512\times512\times(65\textbf{-}764)$ & Thorax CT & Clinical CT & Public & \xmark \\ 

\midrule
FACTS \cite{Bardenfleth_FACTS} & 13 & 26 & $1014 \times 1372 \times 1584$ (mean) & Brain MRI & Lab- \& clinical CT & Public &  \cmark \\ 
WAND \cite{mcnabb2025wand} & 170 & 846 & $\leq 320\times320\times224$ & Brain MRI & T1w, T2w, fMRI, TRUST & Public &  \cmark \\ 
RPLHR-CT \cite{RPLHR_CT} & 250 & 500 & $512 \times 521\times(191\text{-}396)$ & Thorax CT & Clinical CT & On request &  \cmark \\ 
\citet{chu2025paired} & 20 & 40 & $480 \times 512 \times 224$ & Brain MRI & T1w, T2w & Unavailable &  \cmark \\
\citet{li2022deep} & 61 & 122 & $512 \times 512 \times 28$ & Brain MRI & T1w, T2w, FLAIR & On request &  \cmark \\
%LDCT & - & - & $-$ & - & - & Public &  \xmark \\ 
I13-2 XCT \cite{green2025three} & 1 & 4 & $2510\times2510\times2110 $ & Material science & Synchrotron CT & Public &  \cmark \\ 
\citet{solidbattery2023} & 1 & 2 & $ 512 \times 512 \times 200$ & Material science & Lab- \& synchrotron CT & On request &  \cmark \\ 
\citet{klos2025super} & 1 & 6 & $1181\times 1695\times 1695$ (mean) & Material science & Lab-CT & Public &  \cmark \\ 

\midrule
VoDaSuRe & 18 & 36 & $3570 \times 2158 \times 2000$ (mean)\footnote{The volume shape of the samples in VoDaSuRe varies, however all HR scans are chunked in cubes of $160^3$ voxels.}  & Medical \& Material science & Lab- \& synchrotron CT & Public &  \cmark \\ 
\bottomrule
\end{tabular*}
%}%
\end{scriptsize}
\label{tab:ablation_levels}
\end{subtable}

\caption{Overview of image datasets featuring paired volumetric data}
\label{tab:dataset_table}
\end{table*}
%\end{comment}
